MQA-KEAL: Multi-hop Question Answering under Knowledge Editing for Arabic Language

Large Language Models (LLMs) have demonstrated significant capabilities across numerous application domains. A key challenge is to keep these models updated with latest available information, which limits the true potential of these models for the end-applications. Although, there have been numerous attempts for LLMs Knowledge Editing (KE), i.e., to edit the LLMs prior knowledge and in turn test it via Multi-hop Question Answering (MQA), yet so far these studies are primarily focused on English language. To bridge this gap, in this paper we propose: Multi-hop Questioning Answering under Knowledge Editing for Arabic Language (MQA-KEAL). MQA-KEAL stores knowledge edits as structured knowledge units in the external memory. In order to solve multi-hop question, it first uses task-decomposition to decompose the question into smaller sub-problems. Later for each sub-problem, it iteratively queries the external memory and/or target LLM in order to generate the final response. In addition, we also contribute MQUAKE-AR (Arabic translation of English benchmark MQUAKE), as well as a new benchmark MQA-AEVAL for rigorous performance evaluation of MQA under KE for Arabic language. Experimentation evaluation reveals MQA-KEAL outperforms the baseline models by a significant margin.

==> Tab_Fig_tex/old_tab_2_ke.tex <==
\begin{table*}[ht]
{
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{3pt}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lr|ccccc|cccccccc}
% \hline
\toprule
\multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{5}{c|}{\textbf{AecGPT-7B}} & \multicolumn{5}{c}{\textbf{Jais-13B}} \\
% \cline{3-12}
&   
& \textbf{ROME} & \textbf{$\text{MEMIT}$} & \textbf{MEND}  & \textbf{FT-L} & \textbf{SERAC} & \textbf{ROME} & \textbf{$\text{MEMIT}$} & \textbf{MEND}  & \textbf{FT-L} & \textbf{SERAC} \\ 
\midrule
\multirow{4}{*}{\textbf{WikiData$_{recent}$}}  
& Edit Succ. $\uparrow$ & 90.08 & 92.74 & - & 58.23 & 98.76  \\      
& Portability $\uparrow$ & 52.42 & 45.84 & - & 58.22 & 77.34  \\ 
& Locality  $\uparrow$ & 86.49 & 87.18 & - & 77.15 & 85.18  \\ 
& Fluency $\uparrow$ & 432.68 & 427.13 & - & 398.10 & 457.92  \\  \midrule
\multirow{4}{*}{\textbf{ZsRE}}  
& Edit Succ. $\uparrow$ &  89.56 & 85.19 & - & 48.97 & 97.40  \\   
& Portability $\uparrow$ & 54.49 & 54.11 & - & 47.46 & 67.21  \\  
& Locality $\uparrow$   & 74.54 & 83.00 & - & 87.01 & 87.90  \\ 
& Fluency  $\uparrow$ & 419.73 & 423.98 & - & 380.28 & 456.93  \\  \midrule
\multirow{3}{*}{\textbf{WikiBio}}  
& Edit Succ.$\uparrow$  & - & 88.12 & - & 70.81 & 89.49  \\    
& Locality $\uparrow$   & - & 90.98 & - & 92.67 & 97.94  \\ 
& Fluency  $\uparrow$   & - & 588.87 & - & 542.00 & 553.58  \\   \midrule
\multirow{4}{*}{\textbf{WikiData$_{counterfact}$}}  
& Edit Succ. $\uparrow$ & 91.58 & 88.73 & - & 45.96 & 96.35  \\  
& Portability $\uparrow$ & 49.29 & 44.62 & - & 44.07 & 75.39  \\ 
& Locality $\uparrow$ & 85.73 & 91.66 & - & 80.08 & 88.12  \\ 
& Fluency $\uparrow$ & 427.05 & 424.97 & - & 395.69 & 461.03  \\   \midrule
\multirow{3}{*}{\textbf{ConvSent}}  
& Edit Succ. $\uparrow$ & - & 87.44 & - & 66.94 & 97.81 \\                    
% & Portability & \\                            
& Locality $\downarrow$ & - & 0.00 & - & 0.00 & 7494.34  \\ 
& Fluency $\uparrow$ & - & 472.52 & - & 456.42 & 503.23  \\   \midrule
\multirow{3}{*}{\textbf{Sanitation}}  
& Edit Succ. $\uparrow$ & 95.00 & 76.25 & - & 0.00 & -  \\   
& Locality $\uparrow$ & 13.88 & 21.07 & - & 13.30 & -  \\ 
& Fluency $\uparrow$ & 391.14 & 391.14 & - & 391.14 & - \\  \midrule  \midrule 
\multirow{3}{*}{\textbf{ConterFact}}  
& Edit Succ. $\uparrow$ & 88.71 & 92.17 & - & 54.33 & 97.35  \\   
& Locality $\uparrow$ & 97.42 & 97.67 & - & 80.98 & 92.21  \\ 
& Fluency $\uparrow$ & 424.96 & 424.56 & - & 392.83 & 460.81  \\ 
\bottomrule
\end{tabular}
}
}
\caption{Results of existing knowledge edit methods on AceGPT-7B and Jais-13B.
The symbol $\uparrow$ indicates that higher numbers correspond to better performance, while $\downarrow$ denotes the opposite, with lower numbers indicating better performance. WikiData$_{recent}$, ZsRE, WikiBio, WikiData$_{conterfact}$ and Sanitation belong to KnowEdit, and ConterFact is another dataset}
\label{tab:experimental_analysis}
\end{table*}


==> Tab_Fig_tex/tab_res1_MQA_KE_AR.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\resizebox{0.80\linewidth}{!}{%
\begin{tabular}{ll|cccc|cccc|ccc}
\hline
\multicolumn{2}{l}{}                        & \multicolumn{4}{|c|}{\textsc{MQuAKE-CF-ar}} & \multicolumn{4}{c}{\textsc{MquAKE-T-ar}} & \multicolumn{3}{|c}{\OurDATA{}} \\
\multicolumn{2}{l|}{\#Edited Instances}     & 1            & 100          & 1000          & 3000         & 1            & 100          & 500          & 1868         & 1              & 100                    & 229      \\
Large Models & Method                       &              &              &               &              &              &              &              &              &                &                        &          \\
\hline
\jias        & MEMIT                        & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\acegpt      & MEMIT                        & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\gptthree    & MEMIT                        & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
%\gptfour     & MEMIT                        & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\hline
\jias        & MeLLo                        & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\acegpt      & MeLLo                        & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\gptthree    & MeLLo                        & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
%\gptfour     & MeLLo                        & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\hline
\jias        & \OurMODEL{}                  & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\acegpt      & \OurMODEL{}                  & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\gptthree    & \OurMODEL{}                  & x.x          & 25.52\%        & x.x           & x.x          & x.x          & 74.32\%    & 72.51\%          & x.x          & x.x            & x.x                    & x.x      \\
%\gptfour     & \OurMODEL{}                 & x.x          & x.x          & x.x           & x.x          & x.x          & x.x          & x.x          & x.x          & x.x            & x.x                    & x.x      \\
\hline
\end{tabular}%
}
\caption{The result of~\OurMODEL{} for different datasets and target LLMs compared 
against the baseline methods. We report the M-Acc score of~\OurMODEL{}. 
We boldface overall best scores with second best underlined.}
\label{tab:result1_mqaka_ar_old}
\end{table*}

==> Tab_Fig_tex/tab_res1_MQA_KE_AR_bkup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\resizebox{0.80\linewidth}{!}{%
\begin{tabular}{ll|ccc|ccc|ccc}
\hline
\multicolumn{2}{c}{}            & \multicolumn{3}{|c}{\textsc{MQuAKE-CF-ar}} & \multicolumn{3}{|c}{\textsc{MquAKE-T-ar}} & \multicolumn{3}{|c}{\OurDATA{}} \\
Large Models             & Method                       & \textbf{E-Acc}              & \textbf{I-Acc}             & \textbf{M-Acc}            & \textbf{E-Acc}               & \textbf{I-Acc}           & \textbf{M-Acc}             & \textbf{E-Acc}            & \textbf{I-Acc}               & \textbf{M-Acc}              \\
\hline
\multirow{7}{*}{Jias}    & Base                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & FT                           & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MEND                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & ROME                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MEMIT                        & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MeLLo                        & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & \OurMODEL{}                  & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
\hline
\multirow{7}{*}{ACEGPT}  & Base                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & FT                           & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MEND                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & ROME                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MEMIT                        & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MeLLo                        & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & \OurMODEL{}                  & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
\hline
\multirow{7}{*}{GPT-3.5} & Base                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & FT                           & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MEND                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & ROME                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MEMIT                        & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MeLLo                        & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & \OurMODEL{}                  & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
\hline
\multirow{7}{*}{GPT-4o}  & Base                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & FT                           & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MEND                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & ROME                         & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MEMIT                        & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & MeLLo                        & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         & \OurMODEL{}                  & x.x                & x.x               & x.x               & x.x                & x.x              & x.x               & x.x                     & x.x                    & x.x                    \\
                         \hline
\end{tabular}%
}
\caption{Result 2}
\label{tab:result2_mqake_ar}
\end{table*}

==> Tab_Fig_tex/tab_res2_MQA_KE_AR_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\resizebox{0.75\linewidth}{!}{%
\begin{tabular}{ll|ccc|ccc|ccc}
\hline
\multicolumn{2}{l}{}                                                                   & \multicolumn{3}{|c|}{\jias}    & \multicolumn{3}{|c|}{\acegpt}    & \multicolumn{3}{|c}{\gptthree}  \\
Large Models                                            & Method                       & E-Acc     & I-Acc    & M-Acc     & E-Acc     & I-Acc    & M-Acc     & E-Acc     & I-Acc    & M-Acc   \\
\hline
\multirow{7}{*}{\textsc{MQuAKE-CF-ar}}                  & Base                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & -         & 100.0    & x.x      \\
                                                        & FT                           & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MEND                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & ROME                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MEMIT                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MeLLo                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & \OurMODEL{}                  & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        \hline
\multirow{7}{*}{\textsc{MquAKE-T-ar}}                   & Base                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & -         & 100.0    & x.x      \\
                                                        & FT                           & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MEND                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & ROME                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MEMIT                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MeLLo                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & \OurMODEL{}                  & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        \hline
\multirow{7}{*}{\OurDATA{}}                             & Base                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & -         & 99.0     & x.x      \\
                                                        & FT                           & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MEND                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & ROME                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MEMIT                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & MeLLo                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        & \OurMODEL{}                  & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x      \\
                                                        \hline
\end{tabular}%
}
\caption{The results of~\OurMODEL{} compared against the baseline models 
for~\textsc{MQuAKE-CF-ar}  2}
\label{tab:result2_mqake_ar}
\end{table*}




\eat{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\resizebox{0.85\linewidth}{!}{%
\begin{tabular}{ll|ccc|ccc|ccc|ccc}
\hline
\multicolumn{2}{l}{}                                                                   & \multicolumn{3}{|c|}{\jias}    & \multicolumn{3}{|c|}{\acegpt}    & \multicolumn{3}{|c|}{\gptthree}  & \multicolumn{3}{|c}{\gptfour}       \\
Large Models                                            & Method                       & E-Acc     & I-Acc    & M-Acc     & E-Acc     & I-Acc    & M-Acc     & E-Acc     & I-Acc    & M-Acc     & E-Acc     & I-Acc    & M-Acc     \\
\hline
\multirow{7}{*}{\textsc{MQuAKE-CF-ar}}                  & Base                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & FT                           & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MEND                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & ROME                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MEMIT                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MeLLo                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & \OurMODEL{}                  & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        \hline
\multirow{7}{*}{\textsc{MquAKE-T-ar}}                   & Base                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & FT                           & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MEND                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & ROME                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MEMIT                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MeLLo                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & \OurMODEL{}                  & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        \hline
\multirow{7}{*}{\OurDATA{}}                             & Base                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & FT                           & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MEND                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & ROME                         & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MEMIT                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & MeLLo                        & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        & \OurMODEL{}                  & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       & x.x       & x.x      & x.x       \\
                                                        \hline
\end{tabular}%
}
\caption{Result 1}
\label{tab:result1_mqake_ar}
\end{table*}
}

==> commands.tex <==
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{color}
\usepackage{epsfig}
\usepackage{xspace}
\usepackage{graphicx}
%\usepackage{subcaption}
\usepackage{cleveref}
%\usepackage{times}
\usepackage{subfigure}
%\usepackage{cite}
%\usepackage[pdftex]{graphicx}
\usepackage{balance}
\usepackage{hhline}
\usepackage{float}
\usepackage{xcolor}
\usepackage{tabu}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT DELETE!!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%s
%\usepackage{tikz}
%\usetikzlibrary{trees}

\usepackage{epsfig}
\usepackage{multirow}
\usepackage{url}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Enumerate and Itemize modifications
\let\labelindent\relax

\usepackage{enumitem}
\setlist{topsep=0pt,noitemsep} \setitemize[1]{label=$\circ$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\sloppy
\newcommand{\cdd}[1]{|\!|{#1}|\!|}
\newcommand{\cd}[1]{|{#1}|}

\newcommand{\rtable}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\ratt}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\at}[1]{\protect\ensuremath{\mathsf{#1}}\xspace}
\newcommand{\myhrule}{\rule[.5pt]{\hsize}{.5pt}}
\newcommand{\oneurl}[1]{\texttt{#1}}
\newcommand{\eat}[1]{}
\newcommand{\stab}{\rule{0pt}{8pt}\\[-1.2ex]}
\newcommand{\sttab}{\rule{0pt}{8pt}\\[-2ex]}
\newcommand{\sstab}{\rule{0pt}{8pt}\\[-1.7ex]}
\newcommand{\tabstrut}{\rule{0pt}{4pt}\vspace{-0.07in}}
\newcommand{\vs}{\vspace{1.36ex}}
\newcommand{\exa}[2]{{\tt\begin{tabbing}\hspace{#1}\=\+\kill #2\end{tabbing}}}
\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}
%\newcommand{\bi}{\begin{itemize}}
\newenvironment{bi}{\begin{itemize}
        \setlength{\topsep}{1ex}\setlength{\itemsep}{0.6ex}\vspace{0.6ex}}
        {\end{itemize}\vspace{1ex}}
\newcommand{\ei}{\end{itemize}\vspace{1ex}}
\newenvironment{be}{\begin{enumerate}
        \setlength{\topsep}{1ex}\setlength{\itemsep}{0.6ex}\vspace{0.6ex}}
        {\end{enumerate}\vspace{1ex}}
\newenvironment{tbi}{\begin{itemize}\vspace{0.6ex}
        \setlength{\topsep}{1ex}\setlength{\itemsep}{0ex}}
        {\end{itemize}\vspace{-1.5ex}}
\newenvironment{tbe}{\begin{enumerate}\vspace{0.6ex}
        \setlength{\topsep}{0.36ex}\setlength{\itemsep}{0ex}\vspace{0ex}}
        {\end{itemize}\vspace{-1.5ex}}

\newcommand{\A}{{\mathcal A}}
%\newcommand{\C}{{\mathcal C}}
\newcommand{\mat}[2]{{\begin{tabbing}\hspace{#1}\=\+\kill #2\end{tabbing}}}
\newcommand{\m}{\hspace{0.05in}}
\newcommand{\ls}{\hspace{0.1in}}
%\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}\vspace{1ex}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\card}[1]{\mid\! #1\!\mid}
\newcommand{\fth}{\hfill $\Box$}
\newcommand{\AND}{\displaystyle{\bigwedge_{i=1}^{n}}}
%\newcommand{\U}[1]{\displaystyle{\bigcup_{#1}}}
\newcommand{\Sm}[1]{\displaystyle{\sum_{#1}}}
\newcommand{\stitle}[1]{\vspace{1.2ex}\noindent{\bf #1}}
\newcommand{\etitle}[1]{\vspace{1ex}\noindent{\em\underline{#1}}}
\newcommand{\eetitle}[1]{\vspace{1ex}\noindent{\em{#1}}}
\renewcommand{\t}{\tau}
\newcommand{\Inh}[1]{\$#1}
\renewcommand{\r}[1]{{\it rule}(#1)}
\newcommand{\pa}{\parallel}
\newcommand{\LHS}{\kw{{\small LHS}}\xspace}
\newcommand{\knull}{\kw{null}}
\newcommand{\RHS}{\kw{RHS}\xspace}
\newcommand{\ie}{\emph{i.e.,}\xspace}
\newcommand{\eg}{\emph{e.g.,}\xspace}
\newcommand{\st}{\emph{s.t.}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\aka}{\emph{a.k.a.}\xspace}
\newcommand{\kwlog}{\emph{w.l.o.g.}\xspace}
\newcommand{\kwhp}{\emph{w.h.p.}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                  Relation Algebra operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\smallskip}{\vspace{0.6ex}}
\newcommand{\RS}{{\small S}\xspace}
\newcommand{\RA}{\kw{RA}}
\newcommand{\RP}{{\small P}\xspace}
\newcommand{\RJ}{{\sc j}\xspace}
\newcommand{\RC}{{\small C}\xspace}
\newcommand{\RSJ}{{\small SJ}\xspace}
\newcommand{\RSC}{{\small SC}\xspace}
\newcommand{\RSP}{{\small SP}\xspace}
\newcommand{\RPJ}{{\small PJ}\xspace}
\newcommand{\RPC}{{\small PC}\xspace}
\newcommand{\RSPJ}{{\sc spj}\xspace}

\newcommand{\CQ}{\kw{CQ}}
\newcommand{\FO}{\kw{FO}}
\newcommand{\FOC}{\kw{FO[COUNT]}}
\newcommand{\RSPJU}{{\sc spju}\xspace}
%\newcommand{\RSPCU}{{\small SPCU}\xspace}
\newcommand{\RSPJUN}{{\small SPJU$^N$}\xspace}
\newcommand{\RSPCU}{\kw{SPCU}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ALGORITHMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\SELECT}{\mbox{{\bf select}}\ }
\newcommand{\FROM}{\mbox{{\bf from}\ }}
\newcommand{\WHERE}{\mbox{\bf where}\ }
\newcommand{\SUM}{\mbox{{\bf sum}}\ }
\newcommand{\GROUPBY}{\mbox{{\bf group by}}\ }
\newcommand{\HAVING}{\mbox{{\bf having}}\ }
\newcommand{\CASE}{\mbox{{\bf case}}\ }
\newcommand{\END}{\mbox{{\bf end}}\ }
\newcommand{\WHEN}{\mbox{{\bf when}}\ }
\newcommand{\EXISTS}{\mbox{{\bf exists}}\ }
\newcommand{\COUNT}{\mbox{\kw{count}}}
\newcommand{\INSERTINTO}{\mbox{{\bf insert into}}\ }
\newcommand{\UPDATE}{\mbox{{\bf update}}\ }
\newcommand{\SET}{\mbox{{\bf set}}\ }
\newcommand{\IN}{\mbox{{\bf in}}\ }
\newcommand{\If}{\mbox{\bf if}\ }
\newcommand{\Let}{\mbox{\bf let}\ }
\newcommand{\Call}{\mbox{\bf call}\ }
\newcommand{\Then}{\mbox{\bf then}\ }
\newcommand{\To}{\mbox{\bf to}\ }
\newcommand{\Else}{\mbox{\bf else}\ }
\newcommand{\ElseIf}{\mbox{\bf elseif}\ }
\newcommand{\While}{\mbox{\bf while}\ }
\newcommand{\Exists}{\mbox{\bf exists}\ }
\newcommand{\Begin}{\mbox{\bf begin}\ }
\newcommand{\End}{\mbox{\bf end}\ }
\newcommand{\Do}{\mbox{\bf do}\ }
\newcommand{\Downto}{\mbox{\bf downto}\ }
\newcommand{\Repeat}{\mbox{\bf repeat}\ }
\newcommand{\Until}{\mbox{\bf until}\ }
\newcommand{\For}{\mbox{\bf for}\ }
\newcommand{\Each}{\mbox{\bf each}\ }

\newcommand{\ForEach}{\mbox{\bf for each}\ }
\newcommand{\Or}{\mbox{\bf or}\ }
\renewcommand{\And}{\mbox{\bf and}\ }
\newcommand{\Not}{\mbox{\bf not}\ }
\newcommand{\Break}{\mbox{\bf break}}
\newcommand{\Continue}{\mbox{\bf continue}\ }
\newcommand{\Return}{\mbox{\bf return}\ }
\newcommand{\Case}{\mbox{\bf case}\ }
\newcommand{\Of}{\mbox{\bf of}\ }
\newcommand{\EndCase}{\mbox{\bf end-case}\ }
\newcommand{\NIL}{\mbox{\em nil}}
\newcommand{\False}{\mbox{\em false}\xspace}
\newcommand{\True}{\mbox{\em true}\xspace}
\newcommand{\algAND}{{\sc and}\xspace}
\newcommand{\OR}{{\sc or}\xspace}
\newcommand{\NOT}{{\sc not}\xspace}
\newcommand{\kw}[1]{{\ensuremath {\mathsf{#1}}}\xspace}

\newcommand{\false}{\kw{false}}
\newcommand{\true}{\kw{true}}


\newcounter{ccc}
\newcommand{\bcc}{\setcounter{ccc}{1}\theccc.}
\newcommand{\icc}{\addtocounter{ccc}{1}\theccc.}
\newcommand{\preProcessing}{{\mbox{\small\sf preProcessing}\xspace}}
\newcommand{\CFDconsistency}{{\mbox{\small\sf CFD\_Checking}\xspace}}
\newcommand{\MCS} {\kw{MCS}}
\newcommand{\templateDB}{{\mbox{\small\sf templateDB}\xspace}}
\newcommand{\ChaseChecking}{{\mbox{\small\sf RandomChecking}\xspace}}
\newcommand{\chase}{\kw{chase}}
\newcommand{\SAT}{{\mbox{\small\sf SAT}\xspace}}
\newcommand{\kSAT}{{\mbox{\small 3SAT}\xspace}}

\newcommand{\bchk}{\kw{BChk}}
\newcommand{\ebchk}{\kw{EBChk}}
\newcommand{\sebchk}{\kw{sEBChk}}
\newcommand{\findDP}{\kw{FindDP}}
\newcommand{\eval}{\kw{QPlan}}
\newcommand{\seval}{\kw{sQPlan}}
\newcommand{\evalr}{\kw{evalQR}}
\newcommand{\evalh}{\kw{evalQ_{h}}}
\newcommand{\eechk}{\kw{EEChk}}
\newcommand{\seechk}{\kw{sEEChk}}
\newcommand{\optvf}{\kw{optVF2}}
\newcommand{\vf}{\kw{VF2}}
\newcommand{\gsim}{\kw{gsim}}
\newcommand{\optgsim}{\kw{optgsim}}

\newcommand{\PropCFDSPCU}{\kw{Prop{\small CFD\_SPCU}}}
\newcommand{\UnionEQs}{\kw{UnionEQs}}
\newcommand{\UnionCFDs}{\kw{UnionCFDs}}
\newcommand{\EQ}{\kw{EQ}}
\newcommand{\eq}{\kw{eq}}

\newcommand{\rep}{\kw{rep}}
\newcommand{\PEQ}{\kw{EQ2CFD}}
\newcommand{\Drop}{\kw{Drop}}
\newcommand{\Res}{\kw{Res}}
\newcommand{\AR}{{\small AR}\xspace}
\newcommand{\ARs}{{\small AR}s\xspace}
\newcommand{\CFD}{\kw{CFD}}
\newcommand{\CFDs}{\kw{CFDs}}
\newcommand{\CIND}{{\sc cind}\xspace}
\newcommand{\cind}{{\small \sf CIND}}
\newcommand{\cfd}{{\small \sf CFD}}
\newcommand{\CINDp}{{\sc cind}$^+$\xspace}
\newcommand{\CINDn}{{\sc cind}$^-$\xspace}
\newcommand{\CINDs}{\kw{INDs}}
\newcommand{\FD}{\kw{FD}}
\newcommand{\FDs}{\kw{FDs}}
\newcommand{\IND}{{\sc ind}\xspace}
\newcommand{\INDs}{\kw{INDs}}
\newcommand{\BD}{\kw{BD}}
\newcommand{\BDT}{\kw{BDT}_\kw{P}}
\newcommand{\BDTQ}{\kw{BDT}_\kw{Q}}
\newcommand{\DP}{\kw{DP}}
\newcommand{\NP}{\kw{NP}}
\newcommand{\NPC}{\kw{NPC}}
\renewcommand{\P}{\kw{P}}
\newcommand{\klog}{\kw{log}}
\newcommand{\NL}{\kw{NL}}
\newcommand{\SPC}{\kw{SPC}}
\newcommand{\logspace}{\kw{log}-\kw{space}}
\newcommand{\polylogT}{\kw{polylog}-\kw{time}}
\newcommand{\polylogS}{\kw{polylog}-\kw{space}}
\newcommand{\DAGs}{{\small DAG}s\xspace}

\newcommand{\redu}{\leqslant_{\text{\sl fa}}^\NC}
\newcommand{\reduf}{\leqslant_F^\NC}

\newcommand{\GFD}{\kw{GFD}}
\newcommand{\GFDs}{\kw{GFDs}}

\newcommand{\GFDx}{\kw{GFD_x}}
\newcommand{\GFDxs}{\kw{GFD_xs}}

\newcommand{\GED}{\kw{GED}}
\newcommand{\GEDs}{\kw{GEDs}}

\newcommand{\GEDx}{\kw{GED_x}}
\newcommand{\GEDxs}{\kw{GED_xs}}

\newcommand{\key}{\kw{GKey}}
\newcommand{\keys}{\kw{GKeys}}


\newcommand{\GDC}{\kw{GDC}}
\newcommand{\GDCs}{\kw{GDCs}}

\newcommand{\GEDor}{\kw{GED^\lor}}
\newcommand{\GEDors}{\kw{GED^{\lor}s}}

\newcommand{\GEDt}{\kw{GED^\t}}
\newcommand{\GEDts}{\kw{GED^{\t}s}}

\newcommand{\NC}{\kw{NC}}
\newcommand{\coNP}{\kw{coNP}}
\newcommand{\PTIME}{\kw{PTIME}}
\newcommand{\PSPACE}{\kw{PSPACE}}
\newcommand{\EXPTIME}{\kw{EXPTIME}}
\newcommand{\NPSPACE}{\kw{NPSPACE}}
\newcommand{\dom}{\protect\ensuremath{\mathsf{dom}}\xspace}
%\newcommand{\adom}{\protect\ensuremath{\mathsf{Adom}}\xspace}
\newcommand{\atset}{\protect\ensuremath{\mathsf{attr}}\xspace}
\newcommand{\attr}[1]{\protect\ensuremath{\mathsf{#1}}\xspace}
\newcommand{\attrset}{\protect\ensuremath{\mathsf{attr}}\xspace}
\newcommand{\finatset}{\protect\ensuremath{\mathsf{finattr}}\xspace}
\newcommand{\pvar}{\protect\ensuremath{\mathsf{var\%}}\xspace}
\newcommand{\lLHS}{\protect\ensuremath{\mathsf{{\small LHS}}}\xspace}
\newcommand{\RBR}{\kw{RBR}}
\newcommand{\SQL}{\kw{SQL}}
\newcommand{\XSLT}{{\sc xslt}\xspace}
\newcommand{\DBMS}{{\sc dbms}\xspace}
\newcommand{\ATG}{{\sc atg}\xspace}
\newcommand{\ATGs}{{\sc atg}{\small s}\xspace}
\newcommand{\EBI}{{\sc ebi}\xspace}
\newcommand{\GO}{{\sc go}\xspace}
\newcommand{\VEC}[1]{{\sc vec}(#1)}
\newcommand{\DAG}{{\small DAG}\xspace}
\newcommand{\XQ}{{\sc xq}\xspace}
\newcommand{\XQwc}{{\sc xq}$^{\scriptscriptstyle[*]}$\xspace}
\newcommand{\XQdes}{{\sc xq}$^{\scriptscriptstyle[//]}$\xspace}
\newcommand{\XQfull}{{\sc xq}$^{\scriptscriptstyle[*,//]}$\xspace}
\newcommand{\vect}[1]{$\langle$ #1 $\rangle$}
\newcommand{\sem}[1]{[\![#1]\!]}
\newcommand{\NN}[2]{#1\sem{#2}}
\newcommand{\e}[2]{{\mathit (#1,#2)}}
\newcommand{\ep}[2]{{\mathit (#1,#2)+}}
\newcommand{\brname}{\ensuremath{{\mathsf{N}}}}
\newcommand{\budrel}[1]{\ensuremath{{\brname_{#1}}}}
\newcommand{\budgen}[2]{\ensuremath{Q^\brname_\e{#1}{#2}}}
\newcommand{\budcut}[2]{\ensuremath{Q_\e{#1}{#2}}}
%\newcommand{\G}{{\cal G}}
\newcommand{\I}{{\cal I}}
\newcommand{\V}{{\cal V}}
\newcommand{\E}{{\cal E}}

\newcommand{\po}{\preceq}       % for partial order
\newcommand{\spo}{\prec}


\newcommand{\eop}{\hspace*{\fill}\mbox{$\Box$}}     % End of proof
\newcounter{example}%[section]
\renewcommand{\theexample}{\arabic{example}}
\newenvironment{example}{
        \vspace{1.2ex}
        \refstepcounter{example}
        {\noindent\bf Example \theexample:}}{
        \eop\vspace{1.2ex}}
\def\copyrightspace{}
\renewcommand{\ni}{\noindent}
\newcommand{\comlore}[1]{\begin{minipage}{3in}\fbox{\fbox{\parbox[t]{3in}{{\vspace{2mm}\noindent \bf COMM(LORE):~
{ #1}\hfill  END.}}}}\end{minipage}\\}
\newcommand{\comwenfei}[1]{\begin{minipage}{3in}\fbox{\fbox{\parbox[t]{3in}{{\vspace{2mm}\noindent \bf COMM(WENFEI):~
{ #1}\hfill  END.}}}}\end{minipage}\\}
\newcommand{\comshuai}[1]{\begin{minipage}{3in}\fbox{\fbox{\parbox[t]{3in}{{\vspace{2mm}\noindent \bf COMM(SHUAI):~
{ #1}\hfill  END.}}}}\end{minipage}\\}
\newcommand{\nthesection}{\arabic{section}}
\newcounter{theorem}%[section]
\renewcommand{\thetheorem}{\arabic{theorem}}
\newcounter{prop}%[section]
\renewcommand{\theprop}{\arabic{theorem}}
\newcounter{lemma}%[section]
\renewcommand{\thelemma}{\arabic{theorem}}
\newcounter{cor}%[section]
\renewcommand{\thecor}{\arabic{theorem}}
\newenvironment{theorem}{\begin{em}
        \refstepcounter{theorem}
        {\vspace{1ex} \noindent\bf  Theorem  \thetheorem:}}{
        \end{em}\eop\vspace{1ex}} %\hspace*{\fill}\vspace*{1ex}}
\newenvironment{prop}{\begin{em}
        \refstepcounter{theorem}
        {\vspace{1ex}\noindent \bf Proposition \theprop:}}{
        \end{em}\eop\vspace{1ex}}%\hspace*{\fill}\vspace*{1ex}}
\newenvironment{ctheorem}[1]{\begin{em}
        \refstepcounter{theorem}
        {\vspace{1.5ex}\noindent \bf Theorem \theprop~#1:}}{
        \end{em}\eop\vspace{1.5ex}}%\hspace*{\fill}\vspace*{1ex}}
\newenvironment{clemma}[1]{\begin{em}
        \refstepcounter{theorem}
        {\vspace{1ex}\noindent\bf Lemma \thelemma~#1:}}{
        \end{em}\eop\vspace{1ex}} %\hspace*{\fill}\vspace*{1ex}}
\newenvironment{lemma}{\begin{em}
        \refstepcounter{theorem}
        {\vspace{1.5ex}\noindent\bf Lemma \thelemma:}}{
        \end{em}\eop\vspace{1.5ex}} %\hspace*{\fill}\vspace*{1ex}}
\newenvironment{cor}{\begin{em}
        \refstepcounter{theorem}
        {\vspace{1.5ex}\noindent\bf Corollary \thecor:}}{
        \end{em}\eop\vspace{1.5ex}} %\hspace*{\fill}\vspace*{1ex}}
\newcounter{definition}%[section]
\renewcommand{\thedefinition}{\arabic{definition}}
\newenvironment{definition}{
        \vspace{1.5ex}
        \refstepcounter{definition}
        {\noindent\bf Definition {\bf \thedefinition}:}}{\eop\vspace{1.5ex}
}
\newcounter{alg}[section]
\renewcommand{\thealg}{\nthesection.\arabic{alg}}
\newenvironment{alg}[1]{
        \refstepcounter{alg}
        {\vspace{1ex}\noindent\bf Algorithm \thealg:\, #1}}{
        \vspace*{1ex}}
\newcounter{arule}
\renewcommand{\thearule}{\arabic{arule}}
\newenvironment{arule}{
        \vspace{0.6ex}
        \refstepcounter{arule}
        {\noindent \em Rule \thearule:}}{
        }
\newcounter{claim}
\renewcommand{\theclaim}{\arabic{claim}}
\newenvironment{claim}{
        \vspace{0.6ex}
        \refstepcounter{claim}
        {\noindent\em Claim \theclaim:}}{{ Wenfei Fan}\\
        }
\renewenvironment{proof}{
        \vspace{1ex}
        {\noindent\bf Proof:}}{\eop\vspace{1ex}}
\newenvironment{proofS}{
        \vspace{1ex}
        {\noindent\bf Proof sketch:\ }}{\eop\vspace{1ex}}



\renewcommand{\P}{\kw{P}}
\newcommand{\APX}{\kw{APX}}
\newcommand{\PTAS}{{\small PTAS}\xspace}
\newcommand{\FPTAS}{{\small FPTAS}\xspace}
\newcommand{\NPO}{\kw{NPO}}

%\newcommand{\inst}{\protect{\mathsf{inst}}\xspace}
\renewcommand{\lq}{{\cal L}_Q}
\newcommand{\SPCU}{\kw{SPCU}}


\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\bc}{{\cal B}}
\newcommand{\df}{{\cal D}_I}
\newcommand{\imp}{\vdash}
\newcommand{\impq}{\models_{\Gamma,\Sigma}}


\newlist{myitemize}{itemize}{3}
\setlist[myitemize,1]{label=$\circ$,leftmargin=2.6ex}
\setlist[myitemize,2]{label=$\bullet$,leftmargin=3.8ex}
\setlist[myitemize,3]{label=$\diamond$, leftmargin=3.2ex}
\newenvironment{mbi}{\begin{myitemize}
        \setlength{\topsep}{0.8ex}\setlength{\itemsep}{0.36ex}\vspace{0.6ex}}
        {\end{myitemize}\vspace{0.8ex}}
\newenvironment{tmbi}{\begin{myitemize}
        \setlength{\topsep}{0.8ex}\setlength{\itemsep}{0.36ex}\vspace{0.36ex}}
        {\end{myitemize}\vspace{0.8ex}}
\newcommand{\mei}{\end{myitemize}\vspace{0.6ex}}


\newcommand{\bnd}{\kw{Bnd}}
\newcommand{\ebnd}{\kw{EBnd}}
\newcommand{\bndm}{\kw{MBnd}}
\newcommand{\ebndm}{\kw{MEBnd}}

%Dominating problems
\newcommand{\minb}{\kw{DP}}
\newcommand{\mineb}{\kw{DPEB}}
\newcommand{\minbm}{\kw{MDP}}
%\newcommand{\minebm}{$\kw{minEBnd}_M$}
\newcommand{\minebm}{\kw{MDPEB}}
\newcommand{\fdp}{$\kw{findDP_{h}}$\xspace}

\newcommand{\EGD}{\kw{EGD}}
\newcommand{\EGDs}{\kw{EGDs}}
\newcommand{\TGDs}{\kw{TGDs}}

\newcommand{\Vio}{\kw{Vio}}
\newcommand{\DVio}{\kw{Vio}_\Delta}
\newcommand{\Eid}{\kw{Eid}}
%\newcommand{\C}{{\cal C}}
\newcommand{\B}{{\cal B}}
\newcommand{\N}{{\cal N}}

\newcommand{\conflict}{\kw{conflict}}
\newcommand{\closure}{\kw{enforced}}
\newcommand{\Closure}{\kw{closure}}

%\newcommand{\revise}[1]{#1}
\newcommand{\revise}[1]{{\color{black}{#1}}}
\newcommand{\revised}[1]{{\color{black}{#1}}}
\newcommand{\reviseX}[1]{{\color{blue}{#1}}}
%\newcommand{\warn}[1]{#1}
\newcommand{\warnX}[1]{#1}
\newcommand{\warn}[1]{{\color{black}{#1}}}
\newcommand{\iwarn}[1]{{\color{black}{#1}}}
\newcommand{\correct}[1]{{\color{black}{#1}}}
\newcommand{\xie}[1]{{\color{black}{#1}}}
%\newcommand{\todo}{{\color{black}{To do}}}
\newcommand{\wyss}[1]{{\color{black}{#1}}}
\newcommand{\wysss}[1]{{\color{black}{#1}}}
\newcommand{\wys}[1]{{\color{black}{#1}}}
\newcommand{\wysR}[1]{{\color{blue}{#1}}}

\newcommand{\reviseR}[1]{#1}

\newcommand{\warnV}[1]{{\color{black}{#1}}}
\newcommand{\asif}[1]{{\color{black}{#1}}}
%\label{\label{key}}
%\newcommand{\asif}[1]{{\color{violet}{#1}}}


%\newcommand{\newdata}{\kw{Commerce}}
\newcommand{\newdata}{\kw{COM}}
\newcommand{\person}{\kw{Person}}
\newcommand{\critic}{\kw{Critic}}
\newcommand{\gatenc}{$\kw{GATE}_\kw{NC}$\xspace}
\newcommand{\creatoritr}{$\kw{Creator}_\kw{itr}$\xspace}
\newcommand{\creator}{\kw{Creator}}
%\newcommand{\creatorna}{$\kw{Creator}_\kw{NA}$}
\newcommand{\creatornc}{$\kw{Creator}_\kw{NC}$\xspace}
\newcommand{\creatorne}{$\kw{Creator}_\kw{NE}$\xspace}
\newcommand{\creatorna}{$\kw{Creator}_\kw{NA}$\xspace}
\newcommand{\uncertainrule}{\kw{UncertainRule}}
\newcommand{\improvec}{\kw{Improve3C}}
\newcommand{\gateni}{$\kw{GATE}_\kw{NI}$\xspace}
\newcommand{\rankbert}{$\kw{RANK}_\kw{Bert}$\xspace}
\newcommand{\dittorank}{$\kw{Ditto}_\kw{Rank}$\xspace}
\newcommand{\tabnetrank}{$\kw{TabNet}_\kw{Rank}$\xspace}

\newcommand{\lval}{\kw{localVio}}
\newcommand{\fragval}{\kw{fragVal}}

\newcommand{\bqpar}{\kw{bPar}}
\newcommand{\assemble}{\kw{Assemble}}
\newcommand{\dispar}{\kw{disPar}}
\newcommand{\dislval}{\kw{dlovalVio}}
\newcommand{\et}{\kw{et}}
\newcommand{\ec}{\kw{CC}}
\newcommand{\PV}{\kw{PV}}
\newcommand{\reduce}{\kw{reduceW}}
\newcommand{\dist}{\kw{dist}}
\newcommand{\gcfd}{\kw{GCFD}}
\newcommand{\gcfds}{\kw{GCFDs}}


\newcommand{\val}{\kw{detVio}} %% sequential
\newcommand{\repval}{\kw{repVal}} %% replicated
\newcommand{\disval}{\kw{disVal}} %% fragmented
\newcommand{\repran}{$\kw{rep}_{\kw{ran}}$\xspace} %% replicated with random workload assignment
\newcommand{\disran}{$\kw{dis}_{\kw{ran}}$\xspace} %% distributed with random workload assignment
\newcommand{\repnop}{$\kw{rep}_{\kw{nop}}$\xspace} %% replicated with no optimization
\newcommand{\disnop}{$\kw{dis}_{\kw{nop}}$\xspace} %% distributed with no optimization

\newcommand{\pokec}{{\sl Pokec}\xspace}
\newcommand{\yago}{{\sl YAGO2}\xspace}
\newcommand{\dbpedia}{{\sl DBpedia}\xspace}

\newcommand{\gskew}{\kw{skew}}
%\newcommand{\tbf}{\kw{TBF}}

\newcommand{\id}{\kw{id}}

\newcommand{\SEq}{\kw{SEQ}}
\newcommand{\Eq}{\kw{Eq}}
\newcommand{\Eqv}{\kw{Eq}_\varphi}
\newcommand{\Kwlog}{\emph{W.l.o.g.}\xspace}


\newcommand{\LenBound}{2\times (|G|\times |\Sigma|)^2}
%\newcommand{\LenBound}{(|G|\times |\Sigma|)^2 + |G|}

\newcommand{\GGCP}{\kw{GGCP}}
\newcommand{\QGP} {\kw{QGP}}
\newcommand{\QGPs}{\kw{QGPs}}
\newcommand{\GPAR}{\kw{GPAR}}
\newcommand{\GPARs}{\kw{GPARs}}
\newcommand{\GAR}{\kw{QGAR}}
\newcommand{\GARs}{\kw{QGARs}}
% \newcommand{\VP}{\kw{VP}}
% \newcommand{\EP}{\kw{EP}}
\newcommand{\VP}{\Pi_V}
\newcommand{\EP}{\Pi}
\newcommand{\DSIP}{$\kw{DSP}^+$}
\newcommand{\DSOP}{$\kw{DSP}^-$}
\newcommand{\DSVP}{\kw{DSVP}}
\newcommand{\DSEP}{\kw{DSEP}}
\renewcommand{\DSVP}{\kw{DS}}
\renewcommand{\DSEP}{\kw{DSEC}}
\newcommand{\DS}{\kw{DS}}
\newcommand{\DSVC}{\kw{DS}}
\newcommand{\DSEC}{\kw{DSEC}}
\newcommand{\Assemble}{\kw{Assemble}}
\newcommand{\PEval}{\kw{PEval}}
\newcommand{\IncEval}{\kw{IncEval}}
\newcommand{\T}{{\mathcal T}}
\newcommand{\F}{{\mathcal F}}
\newcommand{\M}{{\mathcal M}}
\newcommand{\Mes}{\kw{MSeg}}


\newcommand{\GBSP}{$\AGRAPE_{\BSP}$\xspace}
\newcommand{\GAP}{$\AGRAPE_{\AP}$\xspace}
\newcommand{\GSSP}{$\AGRAPE_{\SSP}$\xspace}
\newcommand{\glabsync}{$\glab_{\kw{sync}}$\xspace}
\newcommand{\glabasync}{$\glab_{\kw{async}}$\xspace}
\newcommand{\BSP}{\kw{BSP}}
\newcommand{\AP}{\kw{AP}}
\newcommand{\SSP}{\kw{SSP}}
\newcommand{\AAP}{\kw{AAP}}

\newcommand{\TTL}{\kw{DS}}
\newcommand{\TIMES}{\kw{X}}
\newcommand{\Q}{{\mathcal Q}}
\newcommand{\PIE}{\kw{PIE}}
\newcommand{\Buff}[1]{{\mathbb{B}_{#1}}}
\newcommand{\GRAPE}{\kw{GRAPE}}
\newcommand{\AGRAPE}{\kw{GRAPE+}}

\newcommand{\HyPar}{\kw{HyPar}}
\newcommand{\HyIncPar}{\kw{HyIncPar}}



\newcommand{\tbf}{\kw{\textcolor{red}{XX}}}
\newcommand{\VC}[1]{#1{-}\textsc{VC}}
\newcommand{\MVC}[1]{\textsc{Min}-#1-\textsc{VC}}

\newcommand{\least}{{\mathcal M}}
\newcommand{\most}{{\mathcal N}}
\newcommand{\ball}{{\mathcal B}}
\newcommand{\range}{{\mathcal L}}
\newcommand{\Ex}{{\bf E}}
\newcommand{\RF}[1]{\partial(#1)}
\newcommand{\etal}{\textit{et al.}}


\makeatletter
\newcommand\figcaption{\def\@captype{figure}\caption}
\newcommand\tabcaption{\def\@captype{table}\caption}
\makeatother



\newcommand{\live}{\kw{liveJournal}}
\newcommand{\traffic}{\kw{traffic}}
\newcommand{\uk}{\kw{UKWeb}}
\newcommand{\friend}{\kw{Friendster}}
\newcommand{\movie}{\kw{movieLens}}
\newcommand{\netflix}{\kw{Netflix}}
\newcommand{\twitter}{\kw{Twitter}}
\newcommand{\syn}{\kw{Synthetic}}

\newcommand{\giraph}{\kw{Giraph}}
\newcommand{\glab}{\kw{GraphLab}}
\newcommand{\blogel}{\kw{Blogel}}
\newcommand{\maiter}{\kw{Maiter}}
\newcommand{\guc}{\kw{GiraphUC}}
\newcommand{\hsync}{\kw{PowerSwitch}}
\newcommand{\petuum}{\kw{Petuum}}
% \newcommand{\PR}{\kw{PageRank}}
\newcommand{\PR}{\kw{PR}}
\newcommand{\CF}{\kw{CF}}

\newcommand{\CH}{\kw{CH}}
% \newcommand{\DBH}{\kw{DBH}}
\newcommand{\DBH}{\kw{Libra}}
\newcommand{\IncP}{\kw{IncP}}
\newcommand{\TDH}{\kw{2DHash}}

\newcommand{\HP}{\ensuremath{\mathsf{HP}}}


\newcommand{\SSSP}{\kw{SSSP}}
\newcommand{\Sim}{\kw{Sim}}
\newcommand{\CN}{\kw{CN}}
\newcommand{\CC}{\kw{CC}}
\newcommand{\CCs}{\kw{CCs}}
\newcommand{\WCC}{\kw{WCC}}
\newcommand{\SG}{{\mathcal S}}


\newcommand{\triList}{\kw{TC}}
\newcommand{\kclique}{\kw{kCList}}
\newcommand{\dijkstra}{\kw{Dijkstra}}
\newcommand{\aggr}{\kw{aggr}}
\newcommand{\BFS}{\kw{BFS}}
\newcommand{\HPP}{\textsf{ADP}}
\newcommand{\HPar}{\kw{HPar}}
\newcommand{\HHPar}{\kw{H2HPar}}
\newcommand{\CExpand}{\textsf{CExpand}}
\newcommand{\CAlloc}{\textsf{CAlloc}}

\newcommand{\PA}{\P_{\!\A}}
\newcommand{\PAH}{\P_{\!\A}^{h}}
\newcommand{\PAG}{\P_{\!\A}^{g}}
\newcommand{\EH}{\textsf{E2H}}
\newcommand{\VH}{\textsf{V2H}}
\newcommand{\ADP}{\textsf{ADP}}
\newcommand{\CAH}{C_{\A}^{h}}
\newcommand{\CAG}{C_{\A}^{g}}

\newcommand{\pulp}{\kw{xtraPuLP}}
\newcommand{\fennel}{\kw{Fennel}}
\newcommand{\dbh}{\kw{Libra}}
\newcommand{\ginger}{\kw{Ginger}}
\newcommand{\NE}{\kw{NE}}


\newcommand{\hpulp}{\kw{HxtraPuLP}}
\newcommand{\hfennel}{\kw{HFennel}}
\newcommand{\hdbh}{\kw{HLibra}}
%\newcommand{\ginger}{\textsf{Ginger}}
\newcommand{\hne}{\kw{HNE}}
\newcommand{\grid}{\kw{Grid}}
\newcommand{\hgrid}{\kw{HGrid}}
\newcommand{\MSRE}{\kw{MSRE}}

\newcommand{\REE}{\kw{REE}}
\newcommand{\REEs}{\kw{REEs}}
\newcommand{\MD}{\kw{MD}}
\newcommand{\MDs}{\kw{MDs}}
\newcommand{\DC}{\kw{DC}}
\newcommand{\DCs}{\kw{DCs}}
\newcommand{\AFF}{\kw{AFF}}
\newcommand{\Ad}{{\mathcal A}_\Delta}

\newcommand{\R}{{\mathcal R}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\W}{{\mathcal W}}
\newcommand{\ids}{\kw{ids}}
\newcommand{\tid}{\kw{tid}}
\newcommand{\pchase}{\kw{PChase}}
\newcommand{\incchase}{\kw{IncChase}}
\newcommand{\BCQE}{\kw{BCQE}}


%%%%%%%%%%%%% REE error detection $$$$$$$$$$$$$$

\newcommand{\REEDet}{\kw{REEDet}}
\newcommand{\HPartition}{\kw{HPartition}}
\newcommand{\PREEDet}{\kw{PREEDet}}
\newcommand{\Leapfrog}{\kw{Leapfrog}}
\newcommand{\WDivide}{\kw{WDivide}}
\newcommand{\Valid}{\kw{Valid}}



\newcommand{\phone}{\kw{phn}}
\newcommand{\createT}{\kw{create\_time}}
\newcommand{\loginT}{\kw{last\_login}}
\newcommand{\location}{\kw{location}}
\newcommand{\tracktime}{\kw{time\_tracked}}
\newcommand{\tnumber}{\kw{number}}
\newcommand{\pay}{\kw{payment}}
\newcommand{\level}{\kw{level}}
\newcommand{\preference}{\kw{preference}}
\newcommand{\plog}{\kw{purchase\_log}}
\newcommand{\account}{\kw{ACCOUNT}}
\newcommand{\mobile}{\kw{MOBILE}}
\newcommand{\idcard}{\kw{ID\_card}}
\newcommand{\product}{\kw{product}}
\newcommand{\buyers}{\kw{buyers}}
\newcommand{\device}{\kw{login\_device}}
\newcommand{\accountV}{\kw{ACCOUNT\_V}}
\newcommand{\predict}{\kw{friend}}
\newcommand{\channels}{\kw{channels}}



\newcommand{\inst}{\kw{ins}}
\newcommand{\delt}{\kw{del}}
\newcommand{\PIncDet}{\kw{PIncDet}}
\newcommand{\IncDet}{\kw{IncDet}}
\newcommand{\CrsVio}{\kw{CrsVio}}
\newcommand{\CrsDet}{\kw{CrsDet}}
\newcommand{\PCrsDet}{\kw{PCrtDet}}
\newcommand{\CrsPar}{\kw{CrsPar}}
\newcommand{\ExtVio}{\kw{ExtVio}}
\newcommand{\CrtVio}{\kw{CrtVio}}
\newcommand{\PCrtDet}{\kw{PCrtDet}}
\newcommand{\Cmp}{\kw{Cmp}}
\renewcommand{\div}{\kw{div}}
\newcommand{\lb}{\kw{BM}}
\newcommand{\extension}{\kw{extn}}
%%
\newcommand{\RDet}{\kw{PREEDet}}
\newcommand{\REECR}{\kw{PCRDet}}
\newcommand{\REEER}{\kw{PERDet}}
\newcommand{\REEML}{\kw{PDet_{nml}}}
%%
\newcommand{\PCRDet}{\kw{PCRDet}}
\newcommand{\PERDet}{\kw{PERDet}}

\newcommand{\tfacc}{\kw{TFACC}}
\newcommand{\PREENH}{{$\kw{PDet}_{\kw{nh}}$}}
\newcommand{\PREEMul}{{$\kw{PDet}_{\kw{mul}}$}}
\newcommand{\PREEDER}{{$\kw{PDet}_{\kw{D}}$}}
\newcommand{\PREERaha}{{$\kw{PDet}_{\kw{R}}$}}

\newcommand{\PIncNH}{{$\kw{PIncDet}_{\kw{nh}}$}}
\newcommand{\PIncMul}{{$\kw{PIncDet}_{\kw{mul}}$}}
%\newcommand{\PREENH}{\kw{PREEDet_{nh}}}
%\newcommand{\PREEMul}{\kw{PREEDet_{mul}}}
%\newcommand{\PIncNH}{\kw{PIncDet_{nh}}}
%\newcommand{\PIncMul}{\kw{PIncDet_{mul}}}
\newcommand{\Holo}{\kw{Holo}}
\newcommand{\DER}{\kw{DER}}
\newcommand{\DMatch}{\kw{DMatch}}
\newcommand{\Raha}{\kw{Raha}}


\newcommand{\HoloD}{\kw{HDet}}
\newcommand{\holoD}{\kw{HDet}}
\newcommand{\scoded}{\kw{SCODED}}
\newcommand{\SCODED}{\kw{SCODED}}
\newcommand{\UClean}{\kw{UClean}}
\newcommand{\Uclean}{\kw{UClean}}
\newcommand{\uclean}{\kw{UClean}}
\newcommand{\ERN}{\kw{ER}-\kw{N}}

\newcommand{\indep}{\perp \!\!\! \perp}
\newcommand{\notindep}{\centernot{\indep}}

%\newcommand{\tfacc}{\kw{TFACC}}
\newcommand{\imdb}{\kw{Movie}}
\newcommand{\house}{\kw{House}}
\newcommand{\tpch}{\kw{TPCH}}

\newcommand{\Fmea}{$F$-\kw{measure}}
\newcommand{\precision}{\kw{Precision}}
\newcommand{\recall}{\kw{Recall}}
\newcommand{\vio}{\kw{Vio}}

\newcommand{\BERT}{\kw{BERT}}


\newcommand{\woc}{$\kw{W}[1]$-complete}
\newcommand{\wh}{$\kw{W}[1]$-hard\xspace}


\newcommand{\GATE}{\kw{GATE}}
\newcommand{\fixme}[1]{\footnote{\textbf{FIXME!!!} #1}} 
\newcommand{\todo}[1]{\textcolor{red}{$\Rightarrow:$ #1}}


